How to detect novelty in textual data streams? A comparative study of existing methods

Since datasets with annotation for novelty at the document and/or word level are not easily available, we present a simulation framework that allows us to create different textual datasets in which we control the way novelty occurs. We also present a benchmark of existing methods for novelty detection in textual data streams. We define a few tasks to solve and compare several state-of-the-art methods. The simulation framework allows us to evaluate their performances according to a set of limited scenarios and test their sensitivity to some parameters. Finally, we experiment with the same methods on different kinds of novelty in the New York Times Annotated Dataset.

==> table/task_3.tex <==


\begin{table}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|} 
\hline
\multicolumn{10}{|c|}{\textbf{Results for task 2 : Detection of new words}} \\
\hline
\hline
\multirow{2}{*}{Methods} & \multicolumn{3}{l|}{Scenario 1}                           & \multicolumn{3}{l|}{Scenario 2}                           & \multicolumn{3}{l|}{Scenario 3}                            \\ 
\cline{2-10}
                         & P                 & R                 & F                 & P                 & R                 & F                 & P                 & R                 & F                  \\ 
\hline
TF-IDF                   & 0                 & 0                 & 0                 & 0.062500          & 0.001832          & 0.003559          & 0.093743          & 0.002781          & 0.005393           \\ 
\hline
BS                       & 0.028670          & 0.005310          & 0.008961          & 0.083396          & 0.013835          & 0.023732          & \textbf{0.125737} & 0.018584          & 0.032381           \\ 
\hline
DF                       & 0                 & 0                 & 0                 & \textbf{0.193268} & 0.052820          & \textbf{0.071080} & 0                 & 0                 & 0                  \\ 
\hline
OLDA                     & 0.029514          & 0.005123          & 0.008730          & 0.084512          & 0.014274          & 0.024422          & 0.109070          & 0.018584          & 0.029744           \\ 
\hline
TopicSketch              & \textbf{0.051119} & \textbf{0.036738} & \textbf{0.040291} & 0.062014          & \textbf{0.056338} & 0.043360          & 0.096412          & \textbf{0.078890} & \textbf{0.083513}  \\
\hline
\hline
\multirow{2}{*}{Methods} & \multicolumn{3}{l|}{Scenario 4}                           & \multicolumn{3}{l|}{Scenario 5}                           & \multicolumn{3}{l|}{Scenario 6}                            \\ 
\cline{2-10}
                         & P                 & R                 & F                 & P                 & R                 & F                 & P                 & R                 & F                  \\ 
\hline
TF-IDF                   & 0.600568          & 0.023128          & 0.04494           & \textbf{0.825462} & 0.055160          & 0.103016          & \textbf{0.856023} & 0.046300          & 0.085869           \\ 
\hline
BS                       & 0.048599          & 0.005592          & 0.010029          & 0.102473          & 0.011002          & 0.019871          & 0.258065          & 0.027642          & 0.049935           \\ 
\hline
DF                       & \textbf{0.638665} & \textbf{0.026925} & 0.050765          & 0.650555          & 0.029941          & 0.056918          & 0.741484          & 0.046583          & 0.087360           \\ 
\hline
OLDA                     & 0.048599          & 0.005592          & 0.010029          & 0.077473          & 0.011002          & 0.019211          & 0.108065          & 0.027642          & 0.043562           \\ 
\hline
TopicSketch              & 0.150755          & 0.096922          & \textbf{0.114037} & 0.165367          & \textbf{0.123100} & \textbf{0.139434} & 0.229587          & \textbf{0.155656} & \textbf{0.183275}  \\
\hline
\hline
\multirow{2}{*}{Methods} & \multicolumn{3}{l|}{Scenario 7}                           & \multicolumn{3}{l|}{Scenario 8}                  & \multicolumn{3}{l|}{Scenario 9}                            \\ 
\cline{2-10}
                         & P                 & R                 & F                 & P                 & R        & F                 & P                 & R                 & F                  \\ 
\hline
TF-IDF                   & \textbf{0.818168} & 0.278367          & 0.375547          & \textbf{0.843606} & 0.167939 & \textbf{0.259563} & \textbf{0.852510} & 0.085783          & 0.149042           \\ 
\hline
BS                       & 0.604651          & \textbf{0.481481} & \textbf{0.536082} & 0.326135          & 0.133379 & 0.189328          & 0.170950          & 0.034744          & 0.057751           \\ 
\hline
DF                       & 0.770845          & 0.054749          & 0.100082          & 0.710740          & 0.071185 & 0.122658          & 0.838778          & 0.052179          & 0.090780           \\ 
\hline
OLDA                     & 0.104651          & 0.181481          & 0.132751          & 0.069421          & 0.080089 & 0.070423          & 0.061188          & 0.045313          & 0.038978           \\ 
\hline
TopicSketch              & 0.216298          & 0.186189          & 0.197154          & 0.209139          & 0.128289 & 0.150002          & 0.221200          & \textbf{0.142328} & \textbf{0.166575}  \\
\hline
\end{tabular}
\end{table}

